Lossless convexification of non-convex optimal control problems with disjoint semi-continuous inputs

This paper presents a convex optimization-based method for finding the globally optimal solutions of a class of mixed-integer non-convex optimal control problems. We consider problems that are non-convex in the input norm, which is a semi-continuous variable that can be zero or lower- and upper-bounded. Using lossless convexification, the non-convex problem is relaxed to a convex problem whose optimal solution is proved to be optimal almost everywhere for the original problem. The relaxed problem can be solved using second-order cone programming, which is a subclass of convex optimization for which there exist numerically reliable solvers with convergence guarantees and polynomial time complexity. This is the first lossless convexification result for mixed-integer optimization problems. An example of spacecraft docking with a rotating space station corroborates the effectiveness of the approach and features a computation time almost three orders of magnitude shorter than a mixed-integer programming formulation.

==> latex_common/preamble.tex <==
% Math
\usepackage{amsmath}
\usepackage{amssymb}
\makeatletter
\@ifclassloaded{autart}{}{\usepackage{amsthm}}
\makeatother
\usepackage{mathtools}
\usepackage{thmtools}
\usepackage{ar}
\usepackage{empheq}
\usepackage{mathrsfs}

\makeatletter
\let\ltxxlabel\ltx@label
\makeatother

% Colors
\usepackage{color}
\makeatletter
\@ifclassloaded{beamer}{}{\usepackage[table]{xcolor}}
\makeatother

% Logic/scripting
\usepackage{ifthen}
\usepackage{pgffor}
\usepackage{etoolbox}
\usepackage{parselines}
\usepackage{environ}
\usepackage{listofitems}
\usepackage{forloop}
\usepackage{calc}
\usepackage{xstring}

% Figures
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{caption}

% Tables
\usepackage{tabularx}
\usepackage{multicol}
\usepackage{diagbox} % \diagbox{rows}{columns} with slash in between
\usepackage{varwidth} % V{max_width} variable-width cell type
\usepackage{makecell} % \makecell[l|r|c]{line 1 \\ line 2}
\usepackage{arydshln}

% Document elements
\usepackage{tikz}
\usepackage[tikz]{mdframed}
% \usepackage{enumitem}
\usepackage{algorithm, algorithmicx}
\usepackage{algpseudocode}%[noend]
\usepackage[many]{tcolorbox}
\usepackage{siunitx}
\usepackage{chemformula}
\usepackage[normalem]{ulem}
\usepackage{accents}
% \usepackage{nicematrix}
% \usepackage{bibentry} % use \bibentry{...} for in-text citation
% \nobibliography*

% Layout
\usepackage{float}
\usepackage{afterpage}
\ifthenelse{\isundefined{\landscapemode}}{
%\usepackage{lscape} % production (non-rotated PDF pages)
%\usepackage{pdflscape} % writing (rotated PDF pages, don't need to twist head)
\def\landscapemode{pdflscape}
}{}
\usepackage{\landscapemode} % writing (rotated PDF pages, don't need to twist head)
\usepackage{varwidth}
\usepackage{nomencl}
\usepackage{longtable}
\usepackage{marginnote}
\makeatletter
\@ifclassloaded{beamer}{}{
\@ifclassloaded{autart}{}{\usepackage{titlesec}}
}
\makeatother
\usepackage{soul}
\usepackage{stackengine}
\usepackage{scalerel}
\usepackage{lastpage}
\usepackage{fancyhdr}

% Referencing
% \usepackage{hyperref}

% General
\usepackage{xspace}

